LLM-Powered Virtual Patient Agents for Interactive Clinical Skills Training with Automated Feedback

Objective Structured Clinical Examinations (OSCEs) are essential for medical training, but they require significant resources, including professional actors and expert medical feedback. Although Large Language Models (LLMs) have introduced text-based virtual patients for communication practice, these simulations often lack the capability for richer, non-textual interactions. This paper presents a novel framework that significantly enhances LLM-based simulated patients by equipping them with action spaces, thereby enabling more realistic and dynamic patient behaviors that extend beyond text. Furthermore, our system incorporates virtual tutors that provide students with instant, personalized feedback on their performance at any time during these simulated encounters. We have conducted a rigorous evaluation of the framework's real-time performance, including system latency and component accuracy. Preliminary evaluations with medical experts assessed the naturalness and coherence of the simulated patients, as well as the usefulness and appropriateness of the virtual tutor's assessments. This innovative system provides medical students with a low-cost, accessible platform for personalized OSCE preparation at home.

==> sections/04_features.tex <==
\section{FEATURES}
\label{sec:use_case}
This section presents a series of usage examples that illustrate the functionality of the framework. A comprehensive list of all prompts can be found in the Supplementary Material. 

\subsection{General System Features}
\textbf{OSCE Scenario Management.} The system allows the creation and management of OSCE scenarios (see Figure~\ref{fig:osce_scenario_management}). To create a scenario for training, it is necessary to provide a patient's \textbf{role description} and a \textbf{task description} for the student. In addition, an \textbf{OSCE checklist} must be provided so that the tutor can perform an evaluation after the training. Training scenarios are stored in the backend and can be updated and modified at any time. 

\subsection{Patient Features}
The first goal of the proposed framework is to enhance the naturalness and coherence of the simulated patient character in training by extending its action capabilities beyond text to include interactive behavior. The following three features illustrate the capabilities of the simulated patient: 

\textbf{Chat Interaction.}
Chat interaction with the simulated patient allows for the practice of communication skills such as taking a patient's history or providing information to the patient. This has also been covered in previous work~\cite{danforth2009development, CampillosLlanos2019DesigningAV}. The student talks to the patient using either voice or text, and responses are returned in the chat. 

\textbf{Movement Behavior.}
By introducing an \textit{action space} of functions in our framework, simulated agents now support interactive movements in addition to pure text-based interaction. To perform an examination, patients can be instructed to move their arms, legs, or joints to certain positions and postures, and the students examine the trajectories. 

\textbf{Reactive Behavior.}
By introducing a \textit{perception space}, an internal state of \textit{observed variables} as well as a \textit{message feed} of the recent history of the interaction, the simulated patient is now capable of reactive behavior with respect to its internal state. For example, a student can change the position of the arm or push the patient's arm in a certain direction. The agent notices this change in position and, when asked, can tell if the movement is painful or not, depending on the medical condition specified. 

\subsection{Tutor Features}
The second goal of the proposed framework is to increase the detail and quality of feedback provided by identifying the steps performed in an OSCE checklist. This extends the keyword matching of existing work to a comprehensive performance assessment that encompasses the entirety of the interaction between the student and the patient agent. The following three features illustrate the capabilities of the tutor agent: 

% Help throughout the Training
\textbf{Interactive Help.}
At any point during a training session, students can ask the tutor for help, such as 'what step to take next'. The tutor is prompted with the patient's role description and knows the task the student is about to perform. In the tutor's role description, the tutor agent is encouraged to respond in a motivating way to help the student figure out how to proceed based on the information given. It is also possible to include additional scenario-related knowledge into the tutor agent prompt to allow for even more detailed case-based support and question-answering. 

% Summary 
\textbf{Training Summary.}
After a training session is completed, the tutor agent provides a detailed summary of the training session. The summary is structured to list positive and negative aspects of the student's performance. Based on the OSCE checklist %the student's role description, and the task description, 
the tutor agent summarizes which checkpoints were appropriately targeted, which were forgotten, or which need to be improved in the future (see Figure~\ref{fig:tutor_training_summary}). By having access to the logs of the entire interaction, the agent can take into account everything that was said or done when summarizing the behavior. This allows for much more fine-grained feedback than a scoring approach that only checks whether certain keywords were used. In addition, by using the LLM's language understanding capabilities, the quality of the conversation can be evaluated much more deeply, allowing students to improve their conversational style and skills with patients. 

% OSCE Score
\textbf{OSCE Score.}
Finally, after the training session has been summarized, the tutor agent distills the evaluation into an OSCE score. To do this, the agent is asked to think through the OSCE checklist step by step~\cite{wei2022chain}. Each successfully completed checklist item is worth 1 point, and each missed item is worth 0 points. The sum of all points is the OSCE score, which gives the student a concrete idea of how well it has performed. The student then knows which scenarios they are good at and which need further study. In contrast to a keyword-matching approach, calculating the OSCE score based on the entire interaction logs and the OSCE checklist has several advantages. First, new training scenarios can be generated very easily by providing only the artifacts \textbf{role description}, \textbf{task description} and \textbf{checklist}, and no hard-coded keyword matching has to be programmed. This makes the training application very \textbf{flexible} and \textbf{extensible}. Second, newly generated training scenarios can be \textbf{automatically evaluated} by LLMs because the language understanding capabilities of LLMs, in combination with the applied step-by-step evaluation procedure, allow them to infer from the context of the conversation whether an OSCE checklist item has been resolved or not. This is much more practical than approaches based on keyword-matching, since keywords may be ambiguous. 

\subsection{Training Session}
% Dynamic Process Example 
The interaction of the simulator frontend with the backend during a training session is illustrated in Figure~\ref{fig:system_architecture_overview}. The user either types or speaks an intended command into the chat component. If the microphone is used, the Whisper speech recognition model transcribes the audio into text. This text is then sent to the appropriate agent API (patient or tutor) in the backend component, depending on which agent is being addressed in the conversation. Once the message is received, the prompt is constructed. The dynamic prompt construction process performed by the \textit{conversation manager} is illustrated in Figure~\ref{fig:osce_system_process_view}. The conversation manager has access to the function sets of the agent's action and perception space. It then filters the stream of logs resulting from the pub-sub mechanism from the simulator for these functions. When a change in the observed variables is detected, the conversation manager updates the observed variables object with those changes (e.g., a change in the position of the arms, legs, or head) and writes them to the prompt. It then adds the last $20$ messages from the filtered log to the prompt to provide the language model with the recent history of the interaction. It also copies the role description and action/perception space functions into the prompt. Finally, the user query is inserted into the prompt. The task given to the LLM is to complete the prompt after the \textit{action::} token with an appropriate function and arguments from the action space. This allows the language model to re-enact the given role and return a function call in JSON format. Once the function call string is generated, it is validated in the backend and then sent to the frontend where it is executed (in this case, the virtual agent in the Unity-based simulator environment). This completes the interaction loop and a new cycle is initiated until the end of the OSCE training session. 

